Speeding up Policy Simulation in Supply Chain RL

Simulating a single trajectory of a dynamical system under some state-dependent policy is a core bottleneck in policy optimization (PO) algorithms. The many inherently serial policy evaluations that must be performed in a single simulation constitute the bulk of this bottleneck. In applying PO to supply chain optimization (SCO) problems, simulating a single sample path corresponding to one month of a supply chain can take several hours. We present an iterative algorithm to accelerate policy simulation, dubbed Picard Iteration. This scheme carefully assigns policy evaluation tasks to independent processes. Within an iteration, any given process evaluates the policy only on its assigned tasks while assuming a certain "cached" evaluation for other tasks; the cache is updated at the end of the iteration. Implemented on GPUs, this scheme admits batched evaluation of the policy across a single trajectory. We prove that the structure afforded by many SCO problems allows convergence in a small number of iterations independent of the horizon. We demonstrate practical speedups of 400x on large-scale SCO problems even with a single GPU, and also demonstrate practical efficacy in other RL environments.

==> Figures/visual_intro.tex <==

\usetikzlibrary{arrows.meta, positioning, shapes.geometric, shadows, backgrounds}



\tikzset{
  timeline/.style={very thick, -Triangle, line cap=round},
  event/.style={rectangle, draw, fill=gray!10!white, text width=2.0cm, text centered, minimum height=1cm, align=center, rounded corners, drop shadow},
  fc/.style args={#1}{circle, draw, thick, fill=#1, minimum size=1cm, align=center, drop shadow},
  label/.style={rectangle, draw=none, fill=none, align=center, minimum height=1cm}
}


\begin{tikzpicture}
  % Draw the timeline
  \draw[timeline] (0,0) -- (14,0);

  % Draw the events on the timeline
  % Event 1 - Product A
  \node[event] (e1) at (2,0) {Product A};
  % Event 2 - Product B
  \node[event] (e2) at (5,0) {Product B};
  % Event 3 - Product A
  \node[event] (e3) at (8,0) {Product A};
  % Event 4 - Product B
  \node[event] (e4) at (11,0) {Product B};

  % Add labels for "Sequential:" and "Parallel:"
  \node[label] (seq) at (0,-2) {\textit{Sequential}:};
  \node[label] (par) at (0,-4) {\textit{Parallel A}:};
  \node[label] (par) at (0,-6) {\textit{Parallel B}:};

  % Draw the FC nodes with shading for "Sequential"
  \node[fc=green!5!white] (fc1) at (2,-2) {FC1};
  \node[fc=green!5!white] (fc2) at (5,-2) {FC1};
  \node[fc=green!5!white] (fc3) at (8,-2) {FC2};
  %\node[fc=green!20!white] (fc4) at (11,-2) {FC2};
  \node[label] (fc4) at (11,-2) {`No fulfill'};

  % Optionally, you can add arrows or lines connecting events to their corresponding FCs
   \draw[->, thick] (e1) -- (fc1);
   \draw[->, thick] (e2) -- (fc2);
   \draw[->, thick] (e3) -- (fc3);
   \draw[->, thick] (e4) -- (fc4);

    % Draw arrows between FC nodes for "Parallel"
    \draw[-> , dotted] (fc1) -- (fc2);
    \draw[-> , dotted] (fc2) -- (fc3);
    \draw[-> , dotted] (fc3) -- (fc4);

   
  % Draw the FC nodes with shading for "Parallel"
  \node[fc=green!5!white] (pfc1) at (2,-4) {FC1};
  %\node[fc=green!30!white] (pfc2) at (5,-4) {FC1};
  \node[fc=red!10!white] (pfc3) at (8,-4) {FC1};
  %\node[fc=red!30!white] (pfc4) at (11,-4) {FC1};

  % Draw the FC nodes with shading for "Parallel"
  %\node[fc=green!30!white] (pfc1) at (2,-6) {FC1};
  \node[fc=green!5!white] (pfc2) at (5,-6) {FC1};
  %\node[fc=red!30!white] (pfc3) at (8,-6) {FC1};
  \node[fc=red!10!white] (pfc4) at (11,-6) {FC1};

    % Draw arrows between FC nodes for "Parallel"
    \draw[-> , dotted] (pfc1) -- (pfc3);
    \draw[-> , dotted] (pfc2) -- (pfc4);

\end{tikzpicture}


==> macros.tex <==

\usepackage[titletoc]{appendix}
\usepackage[final]{microtype}
%\usepackage[ruled]{algorithm2e}
\usepackage{subcaption}
\usepackage{varwidth}
\usepackage{capt-of}
%\usepackage[blocks]{authblk}
\usepackage{boldline}
\usepackage{epsfig}
\usepackage{latexsym}
\usepackage{url}
\usepackage{float}
\usepackage[hidelinks,hypertexnames=false,hyperfootnotes=false]{hyperref}
\usepackage{texnansi}
\usepackage{color}
\usepackage{tikz}
\usepackage{afterpage}
\usepackage{enumerate}
\usepackage[normalem]{ulem}
\usepackage{lmodern}
\usepackage{rotating}
%\usepackage[ruled]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{multicol}
% DS
\usepackage{booktabs}
%
\usepackage{ifthen}
%DS
\usepackage{enumitem}
\setlist[enumerate]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex}


%\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amssymb}
%\usepackage{amsfonts}
% DS 
\usepackage[margin=10pt,font=small,labelfont=bf]{caption}

\usepackage{titlesec}

%deal with the cref issue in PDF bookmarks
%\pdfstringdefDisableCommands{%
%  \def\cref#1{<#1>}%
%}

%\DoubleSpacedXI % Made default 4/4/2014 at request
%\OneAndAHalfSpacedXI % current default line spacing
%%\OneAndAHalfSpacedXII
%%\DoubleSpacedXII

% If hyperref is used, dvi-to-ps driver of choice must be declared as
%   an additional option to the \documentclass. For example
%\documentclass[dvips,opre]{informs3}      % if dvips is used
%\documentclass[dvipsone,opre]{informs3}   % if dvipsone is used, etc.

%%% OPRE uses endnotes. If you do not use them, put a percent sign before
%%% the \theendnotes command. This template does show how to use them.
%\usepackage{endnotes}
%\let\footnote=\endnote
%\let\enotesize=\normalsize
%\def\notesname{Endnotes}%
%\def\makeenmark{$^{\theenmark}$}
%\def\enoteformat{\rightskip0pt\leftskip0pt\parindent=1.75em
%  \leavevmode\llap{\theenmark.\enskip}}

% Private macros here (check that there is no clash with the style)

% Natbib setup for author-year style
%\usepackage{natbib}
% \bibpunct[, ]{(}{)}{,}{a}{}{,}%
% \def\bibfont{\small}%
% \def\bibsep{\smallskipamount}%
% \def\bibhang{24pt}%
% \def\newblock{\ }%
% \def\BIBand{and}%


\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother

%% Setup of theorem styles. Outcomment only one.
%% Preferred default is the first option.
%\TheoremsNumberedThrough     % Preferred (Theorem 1, Lemma 1, Theorem 2)
%\TheoremsNumberedByChapter  % (Theorem 1.1, Lema 1.1, Theorem 1.2)
%\ECRepeatTheorems

%% Setup of the equation numbering system. Outcomment only one.
%% Preferred default is the first option.
%\EquationsNumberedThrough    % Default: (1), (2), ...
%\EquationsNumberedBySection % (1.1), (1.2), ...

% In the reviewing and copyediting stage enter the manuscript number.
%\MANUSCRIPTNO{} % When the article is logged in and DOI assigned to it,
                 %   this manuscript number is no longer necessary

%% useful math macros
\newcommand{\field}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\N}{\ensuremath{\field{N}}} % natural numbers
\newcommand{\R}{\ensuremath{\field{R}}} % real numbers
%\newcommand{\C}{\ensuremath{\field{C}}} % real numbers
\newcommand{\Rp}{\ensuremath{\R_+}} % positive real numbers
\newcommand{\Z}{\ensuremath{\field{Z}}} % integers
\newcommand{\Zp}{\ensuremath{\Z_+}} % positive integers
%\newcommand{\1}{\ensuremath{\mathbf{1}}} % vector of all 1's
%\newcommand{\I}[1]{\ensuremath{\mathbb{I}_{\left\{#1\right\}}}} % indicator function
\newcommand{\Inb}[1]{\ensuremath{\mathbb{I}_{#1}}} % indicator function, no brackets
\newcommand{\tends}{\ensuremath{\rightarrow}} % arrow for limits
\newcommand{\ra}{\ensuremath{\rightarrow}} % abbreviation for right arrow
\newcommand{\PR}{\ensuremath{\mathsf{P}}} % probability
%\newcommand{\E}{\ensuremath{\mathsf{E}}} % expectation
\newcommand{\bbE}{\mathbb{E}} % expectation
\newcommand{\defeq}{\ensuremath{\triangleq}}
\newcommand{\subjectto}{\text{\rm subject to}} % subject to
\renewcommand{\Re}{\ensuremath{\R}} % expectation
%% some caligraphic symbols
\newcommand{\Ascr}{\ensuremath{\mathcal A}}
\newcommand{\Bscr}{\ensuremath{\mathcal B}}
\newcommand{\Cscr}{\ensuremath{\mathcal C}}
\newcommand{\Dscr}{\ensuremath{\mathcal D}}
\newcommand{\Escr}{\ensuremath{\mathcal E}}
\newcommand{\Fscr}{\ensuremath{\mathcal F}}
\newcommand{\Gscr}{\ensuremath{\mathcal G}}
\newcommand{\Hscr}{\ensuremath{\mathcal H}}
\newcommand{\Iscr}{\ensuremath{\mathcal I}}
\newcommand{\Jscr}{\ensuremath{\mathcal J}}
\newcommand{\Kscr}{\ensuremath{\mathcal K}}
\newcommand{\Lscr}{\ensuremath{\mathcal L}}
\newcommand{\Mscr}{\ensuremath{\mathcal M}}
\newcommand{\Nscr}{\ensuremath{\mathcal N}}
\newcommand{\Oscr}{\ensuremath{\mathcal O}}
\newcommand{\Pscr}{\ensuremath{\mathcal P}}
\newcommand{\Qscr}{\ensuremath{\mathcal Q}}
\newcommand{\Rscr}{\ensuremath{\mathcal R}}
\newcommand{\Sscr}{\ensuremath{\mathcal S}}
\newcommand{\Tscr}{\ensuremath{\mathcal T}}
\newcommand{\Uscr}{\ensuremath{\mathcal U}}
\newcommand{\Vscr}{\ensuremath{\mathcal V}}
\newcommand{\Wscr}{\ensuremath{\mathcal W}}
\newcommand{\Xscr}{\ensuremath{\mathcal X}}
\newcommand{\Yscr}{\ensuremath{\mathcal Y}}
\newcommand{\Zscr}{\ensuremath{\mathcal Z}}
%% math operators
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\mean}{mean}
%\DeclareMathOperator{\Var}{Var}
%\DeclareMathOperator{\vect}{vec}
%%\DeclareMathOperator{\vec}{vec}
%\DeclareMathOperator{\interior}{int}
%\DeclareMathOperator{\st}{subject\;to}
%\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
%\DeclareMathOperator*{\argmax}{\mathrm{argmax}}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\minimize}{\ensuremath{\mathop{\mathrm{minimize}}\limits}}
\newcommand{\maximize}{\ensuremath{\mathop{\mathrm{maximize}}\limits}}

%% Misc. new symbols
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\prods}{\calN}
\newcommand{\nprods}{N}
\newcommand{\shelf}{\Mscr}
\newcommand{\shelfcap}{C}
\newcommand{\profit}{p}
\newcommand{\expprofit}{R}
\newcommand{\permgrp}{S}
\newcommand{\sPur}{\calS_j(\shelf)}
\newcommand{\sPurbar}{\overline{\calS}_j(\shelf)}
\newcommand{\sPurd}{\calS_{jd}(\shelf)}
\newcommand{\sPurbard}{\overline{\calS}_{jd}(\shelf)}
\newcommand{\defined}{\overset{\defi}{=}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\co}[1]{\conv \left( #1 \right)}
\newcommand{\Pairs}{\mathcal{P}}
\newcommand{\Triples}{\mathcal{T}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\event}{\mathcal{E}}
\newcommand{\normzero}[1]{\lVert #1 \rVert_{0}}
%\newcommand{\Ee}[1]{{\mathbb E}\left[ #1 \right]}
\newcommand{\abs}[1]{\lvert #1 \rvert}


\newcommand{\hM}{\hat{M}}
\newcommand{\hS}{\hat{S}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hX}{\hat{X}}

\newcommand{\Ln}{\left\|}
\newcommand{\Rn}{\right\|}
\newcommand{\La}{\left\langle}
\newcommand{\Ra}{\right\rangle}

\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\T}{^\intercal}
%\newcommand{\Ber}{{\rm Ber}}
\newcommand{\Uni}{{\rm Uniform}}
\newcommand{\Beta}{{\rm Beta}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%% Tikz customizations
\usetikzlibrary{arrows,patterns,plotmarks}
\tikzstyle{every picture} += [>=stealth]
%% customize section titles
%\allsectionsfont{\sffamily}


\makeatletter
\def\@seccntformat#1{\csname the#1\endcsname.\quad}
\makeatother


% for editing comments
\newcommand{\todo}[1]{{\color{red} \noindent {\sffamily\bfseries TODO:} #1}}

% theorems stated more than once
%\newtheorem*{le:ell}{Lemma~\ref{le:ell}}
%\newtheorem*{le:feas}{Lemma~\ref{le:feas}}
%\newtheorem*{le:sample_complexity}{Lemma~\ref{le:sample_complexity}}
%\newtheorem*{p1}{Proposition~1}
% uncomment to skip figures and compile quickly
%\setboolean{fastcompile}{true}



%\usepackage{setspace}
%\topmargin -0.525in \textwidth 6.5in \textheight 8.75in
%\oddsidemargin 0.0in
%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{subcaption}   %two figures in one line

%\nolinenumbers %disable when submission

\def\draft{1}  % 1 for draft version (eg including author notes), 0 for non-draft version

%---------Fonts---------%
%\usepackage{palatino}
%\usepackage{mathpazo}
%\usepackage{color}
%\usepackage{graphicx}
\usepackage{dsfont}
\usepackage{tcolorbox}


%---------Margins and Length Adjustments---------%
%\usepackage[margin=1in]{geometry}
%\setlength{\parskip}{1em}
%\setlength{\parindent}{0em}
\newcommand{\tinyspace}{\mspace{1mu}}

%---------Math---------%
%\usepackage{amssymb, amsthm, amsmath}
\usepackage{mathtools}

%---------Others--------%
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
%\usepackage{hyperref}
%\hypersetup{
%    colorlinks=true,
%    linkcolor=blue,
%    filecolor=magenta,      
%    urlcolor=cyan,
%}
\usepackage[normalem]{ulem}


%---------Comments-------%
\ifnum\draft=1
\newcommand{\Cr}[1]{{\color{red} #1}}
\newcommand{\Cb}[1]{{\color{blue}#1}}
\else
\newcommand{\Cr}[1]{{#1}}
\newcommand{\Cb}[1]{{#1}}
\fi

%-------- Time ----------%
\newcommand{\notedate}[1]{\hfill \emph{#1}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\def\<{\langle}
\def\>{\rangle}
\def\N{\mathbb{N}}
\def\Nwz{\mathbb{N}_0}
\def\Q{\mathbb{Q}}
\def\C{\mathbb{C}}
\def\R{\mathbb{R}}
\def\eps{\varepsilon}
\newcommand{\fid}{\operatorname{F}}
%\newcommand{\h}{\mathcal{H}}
\newcommand{\norm}[1]{\left\lVert\mspace{1mu} #1 \mspace{1mu}\right\rVert}

\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[3]{\langle #1|#2|#3\rangle}
%%inner product
\newcommand{\ip}[2]{\langle #1|#2\rangle}
%%outer product
\newcommand{\op}[2]{|#1\rangle \langle #2|}
\newcommand{\symm}[1]{{\mathfrak S}_{#1}}
\newcommand{\unitary}[1]{U_{#1}}
\newcommand{\srep}{{\mathtt P}}
\newcommand{\urep}{{\mathtt Q}}

\newcommand{\tr}{{\rm tr}}
\newcommand{\trx}[1]{{\rm tr \left[#1\right]}}
%\newcommand{\mod}{{\rm mod}}
\newcommand{\E}[1] {{\mathbb{E}}\left(#1\right)}
\newcommand{\Ex}[2] {{\mathbb{E}}_{#1}\left(#2\right)}
\newcommand {\Prob}[1] {{\mathbb{P}}\left(#1\right)}
\newcommand {\Probx}[2] {{\mathbb{P}}_{#1}\left(#2\right)}

\newcommand {\sgn} {\mathrm{sgn}}

\newcommand {\F } {{\mathrm{F}}}
\newcommand {\diag } {{\rm diag}}
\newcommand {\Ber} {{\rm Ber}}
\newcommand {\1}[1] {{\mathds{1}}\left\{#1\right\}}

\newcommand{\ideal}{\mathrm{ideal}}
\newcommand{\TPR}{\mathrm{TPR}}
\newcommand{\FPR}{\mathrm{FPR}}
\newcommand{\Ps}{\mathcal{P^{*}}}
\newcommand{\Ano}{\mathrm{Anom}}
\newcommand{\Pos}{\mathrm{Poisson}}
\newcommand{\SVD}{\mathrm{SVD}}
\newcommand{\AD}{\mathrm{EW}}
\newcommand{\PAD}{\mathcal{P}^{\mathrm{EW}}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\LL}{\mathrm{L}}
\newcommand{\RR}{\mathrm{R}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\A}{\mathrm{A}}

%\DeclareMathOperator*{\minimize}{minimize}

\usepackage{thmtools, thm-restate}
\renewcommand{\H}{\mathrm{H}}
\usepackage[capitalise]{cleveref}

\newcommand{\bmatr}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}

\crefname{assumption}{Assumption}{Assumptions}
\Crefname{assumption}{Assumption}{Assumptions}

\newtheorem{assumption}{Assumption}

%% theorem environments
%\newtheoremstyle{thm-sf}{}{}{\itshape}{}{\sffamily\bfseries}{.}{ }{}
%\theoremstyle{thm-sf}
%\newtheorem{remark}{Remark}
%\newtheorem{assumption}{Assumption}
%\newtheorem{condition}{Condition}
%\newtheorem{definition}{Definition}
%\newtheorem{example}{Example}
%\newtheorem{theorem}{Theorem}
%\newtheorem{conjecture}{Conjecture}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{theorem*}{Theorem}
%\newtheorem{fact}{Fact}
%\newtheorem{observation}{Observation}
%\newtheorem{claim}{Claim}
%\newtheorem*{claim*}{Claim}
%\newtheorem{proposition}{Proposition}
%\newtheorem*{proposition*}{Proposition}
%\newtheorem{informal-theorem}{Theorem}
%\newtheorem{informal-proposition}{Proposition}

%\declaretheorem{claim}
%\declaretheorem{lemma}
%\declaretheorem{theorem}

%

%\newtheorem*{claim-not-low-rank-condition}{Claim}[1]

%\newcommand{\qedsymbol}{\ensuremath{\blacksquare}}

%\renewcommand{\proofname}{{\normalfont\sffamily\bfseries Proof}}
%\renewcommand{\proofname}[1]{{\normalfont\sffamily\bfseries #1}}

%\newenvironment{myproof}[1][\proofname]{%
%  \proof[\normalfont\sffamily\bfseries #1]%
%}{\endproof}

\newcommand{\cc}{\mathrm{c}}
\crefname{assumption}{Assumption}{Assumptions}
\Crefname{assumption}{Assumption}{Assumptions}

